LMOD: A Large Multimodal Ophthalmology Dataset and Benchmark for Large Vision-Language Models

The prevalence of vision-threatening eye diseases is a significant global burden, with many cases remaining undiagnosed or diagnosed too late for effective treatment. Large vision-language models (LVLMs) have the potential to assist in understanding anatomical information, diagnosing eye diseases, and drafting interpretations and follow-up plans, thereby reducing the burden on clinicians and improving access to eye care. However, limited benchmarks are available to assess LVLMs' performance in ophthalmology-specific applications. In this study, we introduce LMOD, a large-scale multimodal ophthalmology benchmark consisting of 21,993 instances across (1) five ophthalmic imaging modalities: optical coherence tomography, color fundus photographs, scanning laser ophthalmoscopy, lens photographs, and surgical scenes; (2) free-text, demographic, and disease biomarker information; and (3) primary ophthalmology-specific applications such as anatomical information understanding, disease diagnosis, and subgroup analysis. In addition, we benchmarked 13 state-of-the-art LVLM representatives from closed-source, open-source, and medical domains. The results demonstrate a significant performance drop for LVLMs in ophthalmology compared to other domains. Systematic error analysis further identified six major failure modes: misclassification, failure to abstain, inconsistent reasoning, hallucination, assertions without justification, and lack of domain-specific knowledge. In contrast, supervised neural networks specifically trained on these tasks as baselines demonstrated high accuracy. These findings underscore the pressing need for benchmarks in the development and validation of ophthalmology-specific LVLMs.

==> sections/ethic.tex <==
% \input{sections/tables/licences}

% \vspace{-8pt}
\section{Ethical and Risk Considerations}
% \vspace{-8pt}
We place a high priority on patient privacy by exclusively using open-access datasets in our study, ensuring that there are no concerns related to privacy leakage. All datasets employed in our research are openly accessible and licensed under various Creative Commons (CC) licenses, allowing for ethical and transparent use. 
% For clarity and transparency, we provide a comprehensive list of the licenses associated with each dataset used in our study in Table \ref{tab:license}. 
For future work involving private data, we will implement strict protocols to prevent data retention and adhere to relevant regulations and ethical guidelines. Any collaborations with healthcare institutions will involve robust data sharing agreements and security measures.

Additionally, to mitigate potential biases in datasets and model performance across diverse populations, we have collected datasets that represent a wide range of ethnicities, including Hispanic, Indian, Austrian, and others. By incorporating data from various populations, we aim to ensure that our models are representative of diverse individuals. However, we acknowledge that biases may still persist, and when deploying our method in real-world settings, it is crucial to collect a comprehensive test dataset that includes diverse ethnicities and other factors to thoroughly validate the model's performance and identify any potential biases. We remain committed to ongoing efforts to ensure dataset diversity and fairness in our research.

% Furthermore, we emphasize that our proposed method is designed to assist and support medical professionals, rather than replace them. We acknowledge the indispensable role of human expertise in healthcare and believe that AI tools should complement, not replace, the knowledge and judgment of trained clinicians. Our approach aims to provide valuable insights and guidance, empowering doctors to make more informed decisions with the help of advanced data analysis and pattern recognition capabilities. However, the final diagnosis and treatment plan should always be determined by the medical professional, whose experience and understanding of the patient’s unique context are essential. In real-world clinical settings, AI should act as a trusted assistant, offering reliable insights that enhance healthcare accuracy and efficiency, while preserving the clinician’s central role.

==> sections/tables/licences.tex <==
\begin{table}
\centering
\resizebox{0.35\textwidth}{!}{
\begin{tabular}{c|c}
\toprule
\textbf{Dataset} & \textbf{Copyright License} \\ 
\midrule 
Cataract-1k & CC BY 4.0 \\ \hline
CAU001 & CC BY 4.0 \\ \hline
G1020 & CC BY-NC 4.0 \\ \hline
Harvard-FairSeg & CC BY-NC-ND 4.0 \\ \hline
IDRID & CC BY 4.0 \\ \hline
OIMHS & CC BY 4.0 \\ \hline
ORIGA & CC BY 4.0 \\ \hline
REFUGE & CC BY 4.0 \\ \hline
Cataract Detection 2 & CC BY 4.0 \\ 
\bottomrule 
\end{tabular}
}
% \vspace{-2mm}
\captionsetup{font=scriptsize}
\caption{Summary of copyright licenses for various publicly available ophthalmology datasets used in \dataset. }
\label{tab:license}
\vspace{-5mm}
\end{table}

==> sections/tables/table_finetune.tex <==
\begin{table}[ht]
    \centering
    \resizebox{0.48\textwidth}{!}{
        \begin{tabular}{lcccccc}
        \toprule
        & \multicolumn{4}{c}{\textbf{Anatomical Recognition}} & \multicolumn{2}{c}{\textbf{Diagnosis Analysis}} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-7}
        \textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{HR} & \textbf{Glaucoma} & \textbf{MH Stage} \\
        \midrule
        Finetuned & Invalid & Invalid & Invalid & Invalid & Invalid & Invalid \\
        \bottomrule
        \end{tabular}
    }
    \caption{\scriptsize Performance of LLaVA-Med-Finetuned on anatomical recognition and diagnosis analysis tasks. The model produced invalid outputs across both tasks.}
    \label{tab:llava_invalid_results}
\vspace{-5pt}
\end{table}

==> sections/tables/table_rej_ratios.tex <==
\begin{table}
  \centering
  \vspace{-3mm}
  \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{l|rr|rr}
    \toprule
     & \multicolumn{2}{c|}{\textbf{Demographics Extraction}} & \multicolumn{2}{c}{\textbf{Diagnosis Analysis}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
    \multirow{-2}{*}{\textbf{Model}} & Age Group (\%) & Sex (\%) & MH Stage (\%) & Glaucoma (\%) \\
    \midrule
    GPT-4o~\cite{2023_openai_gpt4} & 78.71 & 99.90 & 1.31 & 63.69 \\
    LLaVA-Med~\cite{2024_neurips_llavamed} & 0.00 & 0.00 & 0.00 & 0.00 \\
    LLava-v1.5-7b~\cite{2024_neurips_llava} & 12.50 & 0.00 & 0.00 & 0.00 \\
    LLaVA-v1.6-Mistral-7B~\cite{2024_neurips_llava} & 52.36 & 0.00 & 93.42 & 0.00 \\
    LLaVA-v1.6-Vicuna-7B~\cite{2024_neurips_llava} & 100.00 & 0.00 & 100.00 & 0.00 \\
    LLaVA-v1.6-13B~\cite{2024_neurips_llava} & 74.32 & 0.00 & 100.00 & 0.00 \\
    Yi-6B~\cite{2024_yi} & 3.37 & 0.00 & 0.00 & 0.00 \\
    InternVL Chat 2B V1.5~\cite{2024_internvl_cvpr} & 83.78 & 0.00 & 0.00 & 0.00 \\
    InternVL Chat 4B V1.5~\cite{2024_internvl_cvpr} & 0.00 & 0.00 & 0.00 & 0.00 \\
    Qwen~\cite{bai2023qwen} & 0.00 & 0.00 & 0.00 & 0.00 \\
    VILA-1.5-3B~\cite{2023_vila} & 45.00 & 4.49 & 7.89 & 0.00 \\
    VILA-1.5-3B-S2~\cite{2023_vila} & 98.31 & 1.35 & 13.15 & 0.00 \\
    VILA-1.5-8B~\cite{2023_vila} & 2.70 & 0.00 & 6.57 & 0.00 \\
    \bottomrule
    \end{tabular}
    }
\vspace{-1mm}
\captionsetup{font=footnotesize}
\caption{Rejection rates (\%) of LVLMs for out-of-domain queries related to demographics and diagnosis.}
\label{tab:ref_ratios}  % Label is added here
\vspace{-3mm}
\end{table}

